Polymorphic Records for Dynamic Languages

We define and study "row polymorphism" for a type system with set-theoretic types, specifically union, intersection, and negation types. We consider record types that embed row variables and define a subtyping relation by interpreting types into sets of record values and by defining subtyping as the containment of interpretations. We define a functional calculus equipped with operations for field extension, selection, and deletion, its operational semantics, and a type system that we prove to be sound. We provide algorithms for deciding the typing and subtyping relations. This research is motivated by the current trend of defining static type system for dynamic languages and, in our case, by an ongoing effort of endowing the Elixir programming language with a gradual type system.

==> app-models.tex <==
In this section we give the detailed technical development to define
our subtyping relation.

To interpret record values we follow~\citet{frisch04} and represent
a record value by a quasi-constant function that maps labels into
either values
(i.e., the elements of $\Domain$) or $\Undef$. Quasi-constant
functions are total functions that map all but a finite set of elements of their
domain into the same value (called default value). Thus record values
can be represented by quasi-constant functions whose default value is
$\Undef$ (see~\citet{castagna23a} for a more detailed explanation). Formally, let us write  $\Domain_\Undef$ for
$\Domain\cup\{\Undef\}$  where $\Undef$ is a distinguished element not in
$\Domain$. We represent our record values as quasi-constant functions
from $\Labels$ to $\Domain_\Undef$ and, thus, interpret record types
as sets of these functions.

The formal definition of quasi-constant function has been given in
\cref{def:qcf} and repeated below for convenience.

\begin{definition}[\cite{frisch04}]%\label{def:qcf}
Let $Z$ denote some set, a function $r:\Labels\to Z$ is
\emph{quasi-constant} if there exists $z\in Z$ such that the set
$\lbrace\ell{\in}\Labels\mid r(\ell)\not=z\rbrace$ is finite.
%% ; in this case
%% we denote this set by $\dom r$  (i.e., the \textbf{dom}ain of
%% $r$) and the element $z$ by
%% $\textup{\textsf{def}}(r)$ (i.e., the \textbf{def}ault value of $r$).
We use $\Labels\qcfun Z$ to denote
the set of quasi-constant functions from $\Labels$ to $Z$ and the
notation $\qcf{\ell_1=z_1, \ldots,\ell_n=z_n,\,\wild=z}$ to denote the
quasi-constant function $r:\Labels\qcfun Z$ defined
by $r(\ell_i)=z_i$ for $i=1..n$ and $r(\ell)=z$ for
$\ell\in\Labels{\setminus}\lbrace\ell_1,\ldots,\ell_n\rbrace$.
\end{definition}
%% \loic{Problème : ici on définit dom(r) autrement que dans la définition de
%% $\Domain$ (on ne se sert pas de cette version plus tard). On peut aussi éviter d'introduire (def(r)).}
Although this
notation is not univocal (unless we require $z_i\not=z$ and the $\ell_i$'s to be pairwise distinct), this is largely sufficient for the
purposes of this work. If $(Z_\ell)_{\ell\in\Labels}$ is a family of
subsets of $Z$ indexed by \Labels, we denote by
$\prodc{\ell{\in}\Labels}Z_\ell$ the subset of
$\Labels\qcfun Z$ formed by all quasi-constant functions $r$ such that
$r(\ell)\in Z_\ell$ for all $\ell\in\Labels$ (intuitively,
$\prodc{\ell{\in}\Labels}Z_\ell$ is a ``type'' of quasi-constant functions).


Next we have to give an interpretation for the
variables. \citet{castagna11} tell us that type variables must be
interpreted as sets in the domain $\Domain$. Therefore, an
interpretation for type variables is a function in
$\typeVars \to \Pd(\Domain)$. Field variables are not much harder,
since the only difference with type variables is that their
interpretation can contain $\Undef$, and therefore it is a function in
$\fldVars \to \Pd(\Domain_\Undef)$. More difficult is the
interpretation of row variables, since these are mapped
into \emph{rows}, that is, \emph{partial} quasi-constant functions on
$\Labels$. Let us write 
$\Labels \pqcfun \Domain_\Undef$ for the partial quasi-constant
functions from $\Labels$ to $\Domain_\Undef$. Thus, an interpretation
of row variables must map an element of $\rowVars$ into a set of functions in $\Labels \pqcfun \Domain_\Undef$. However, for a
given $\rho$ we cannot consider any element in
$\Pd(\Labels \pqcfun \Domain_\Undef)$: we need that the functions in
the interpretation of $\rho$ are total on $\dom(\rho)$. Formally, we
have:
\begin{definition}[Well-Kinded Interpretation]
Let $\eta$ be a function in
$\rowVars \to \Pd(\Labels \pqcfun \Domain_\Undef)$. We say that $\eta$
is \emph{well kinded} if for every $\rho\in\rowVars$ and for every
$f\in\eta(\rho)$, $f$ is a (total) quasi-constant function in
$\dom(\rho)\qcfun \Domain_\Undef$. We denote by
$\rowVars \wkfun \Pd(\Labels \pqcfun \Domain_\Undef)$ the set of
well-kinded functions.
\end{definition}
In conclusion our interpretation of types will be parametric in an assignment $\eta$ for the variables, which will be a function in  \[
  \etaInter \eqdef (\typeVars \to \Pd(\Domain))
  \cup (\fldVars \to \Pd(\Domain_\Undef))
  \cup (\rowVars \wkfun \Pd(\Labels \pqcfun \Domain_\Undef))
\]

The next step is to define the domain $\Domain$ in which to give
the interpretation of types. This is quite simple for us since it suffices to take the
model defined by~\citet{castagna11} and replace products by
quasi-constant functions. The hard problem for defining this model, and
thus the interpretation of types, is to give an interpretation of the
function spaces, but this problem was solved by~\citet{frisch08} whose
solution is 
reused by~\citet{castagna11}. In a nutshell we want to define an
interpretation function
$\TypeInter .: \Types\to\etaInter\to\Pd(\Domain)$. Since the elements of
$\Domain$ represent the values of the language, then $\Domain$ must
contain the set $\Constants$ of constants of the language, the quasi-constant functions (to represent
record values), and the functions
from $\Domain$ to $\Domain$, but the last containment is impossible for cardinality
reasons. The solution by~\cite{frisch08} is to associate to every
domain $\Domain$ and function  $\TypeInter .: \Types\to\etaInter\to\Pd(\Domain)$ a unique
\emph{extensional interpretation}
$\ExtInter(\cdot): \Types \to \etaInter \to \Pd(\ExtInter_\Domain)$
which fixes the semantic of the type constructors, and then to accept as a valid
interpretation of the types only the pairs  $(\TypeInter .,\Domain)$
such that for all $\eta$, $\TypeInter{t}_\eta=\emptyset\iff\ExtInter(t)_\eta=\emptyset$. 

We invite the reader to refer to \citet[Section 2.2]{castagna11} for a
more detailed explanation of how the extensional interpretation
works and to \citet{frisch08} for full details. Henceforth, we just present
how to extend the extensional interpretation of \citet{castagna11} to
include quasi-constant functions and the interpretation of
row-variables, and pinpoint the differences between the two definitions.
We suppose to be given an interpretation
$\ConstantsInBasicType:\Basics\to\Pd(\Constants)$ of basic types into
sets of constants. Given a set $S$ we use the notation $\overline S$
to denote its complement in an appropriate universe: this notation is in particular used for the
set
%\raisebox{-.5pt}{$\Pd(\overline{\TypeInter{t_1}\times\overline{\TypeInter{t_2}}})$}
\raisebox{-.5pt}{$\Pd(\overline{\parbox[][10.7pt][c]{48pt}{$\TypeInter{t_1}_\eta\times\overline{\parbox[][8.8pt][c]{18pt}{$\TypeInter{t_2}_\eta$}}$}}\,)$}
 which corresponds to interpreting the elements in $t_1\to t_2$ as
binary relations, namely as elements of the set $\{\ f\subseteq\Domain^2\mid \text{for all }(d_1,d_2){\in}f , \text{ if } d_1{\in}\TypeInter{t_1}_\eta\text{ then } d_2{\in}\TypeInter{t_2}_\eta\ \}$.



%% The intuition on the semantics of records is conveyed by the following
%% interpretation of types, that is parametrized by an assignment $\eta$ of
%% variables.
%% For that assignment, we consider cofinite quasi-constant functions.
%% We write $\Labels \qcfun \Domain_\Undef$ the set of total quasi-constant functions from
%% $\Labels$ to $\Domain_\Undef$,
%% where $\Undef$ is an element not in $\Domain$, and use
%% $\Labels \pqcfun \Domain_\Undef$ for partial ones.
%% We will put tags on elements of the domain, and the constant part of the
%% quasi-constant function will map to elements $\Undef^\emptyset$.
%% We suppose that for each $\rho$ all the elements of $\eta(\rho)$ are of domain
%% $\dom(\rho)$, so that $\eta$ assigns to a variable $\rho$ a set of functions in
%% $\dom(\rho) \qcfun \Domain_\Undef$ (and not in $\dom(\rho) \qcfun
%% \Pd(\Domain_\Undef)$).
%% \loic{Attention pour l'interprétation des rows les fonctions ne sont pas
%% totales.}
%% The interpretation $\eta$ is in \[
%%   \etaInter \eqdef (\typeVars \to \Pd(\Domain))
%%   \cup (\fldVars \to \Pd(\Domain_\Undef))
%%   \cup (\rowVars \to \Pd(\Labels \qcfun \Domain_\Undef))
%% \]


%% \begin{definition}[Extensional interpretation]
%%   \label{d:extint}
%%   Let $\Domain$ be a set of elements.  The \emph{extensional domain}
%%   of $\Domain$ is defined as:
%%   \(
%%     \ExtInter_\Domain
%%     = \Constants + \Domain + \Pd(\Domain \times \Domain_\Omega)
%%     + (\Labels \qcfun \Domain_\Undef)
%%   \)
%%   where $\Omega$ and $\Undef$ are two different distinguished elements not in $\Domain$.

%%   Let $\IntQ{\TypeInter{\cdot}}: \Types \to \etaInter \to \Pd(\Domain)$ and
%%   $\IntQF{\TypeInter{\cdot}}: \Types_\Undef \to \etaInter \to \Pd(\Domain_\Undef)$
%%   be set-theoretic interpretations.
%%   The associated \emph{extensional interpretation} of types is the unique function
%%   $\ExtInter(\cdot): \Types \to \etaInter \to \Pd(\ExtInter_\Domain)$
%%   such that:
%%   \beppe{Probleme: $\IntQF{\TypeInter{\cdot}}$ n'apparait pas dans la
%%   definition, seulement $\IntF{\TypeInter{\cdot}}$}
%%   \loic{J'avais fait une typo}

%% \noindent
%%    \(\begin{array}{rl}
%%     \ExtInter(\Empty)
%%     &= \emptyset \\
%%     \ExtInter(\alpha)_\eta
%%     &= \eta(\alpha) \\
%%     \ExtInter(b)_\eta
%%     &= \ConstantsInBasicType(b)\\
%%     \ExtInter(\neg t)_\eta
%%     &= \ExtInter_\Domain \setminus \ExtInter(t)_\eta\\
%%     \ExtInter(t_1 \lor t_2)_\eta
%%     &= \ExtInter(t_1)_\eta \cup \ExtInter(t_2)_\eta\\
%%     \ExtInter(t_1 \to t_2)_\eta
%%     &= \Pd(\overline{\IntQ{\TypeInter{t_1}_\eta} \times
%%     \overline{\IntQ{\TypeInter{t_2}_\eta}}})
%%     \end{array}
%%     \begin{array}{rl}
%%     \ExtInter(\R)_\eta
%%     = \left\{
%%       \begin{array}{ll}\bigcup_{\drow \in \eta(\rho)}
%%          \left(\prod_{\ell \in \fin(\R)} \IntQF{\TypeInter{\R(\ell)}}_\eta \pfconcat \drow \right)
%%     &\text{if $\tail(\R) = \rho$}\\
%%       \prod_{\ell \in \Labels} \IntQF{\TypeInter{\R(\ell)}}_\eta &\text{otherwise}
%%       \end{array}\right.
%%       \end{array}
%% \)
%% \end{definition}
%% \beppe{Pour moi la definition ci-dessous ne fait pas de sens, car
%%     minimum il faudrait demander que les deux interpretations
%%     coincident sur les types. Voici ma definition, qui demande que les
%%     field-types soyent definis de manière inductive (ce qui est
%%     raisonnable)}
%% \loic{Je comprends pas trop où est-ce que ça ne va pas. Les field-types sont
%%   déjà définis de manière inductive grâce à $\IntQF{\TypeInter{\cdot}}$
%%   (\cref{def:indinteta} de la même manière que la façon que tu proposes de la
%%   même façon que les types.}
\begin{definition}[Extensional interpretation]
  \label{d:extint}
  Let $\Domain$ be a set.  The \emph{extensional domain}
  of $\Domain$ is defined as:
  \(
    \ExtInter_\Domain
    = \Constants + \Domain + \Pd(\Domain \times \Domain_\Omega)
    + (\Labels \qcfun \Domain_\Undef)
  \)
  where $\Omega$ and $\Undef$ are two different distinguished elements not in $\Domain$.

  Let $%\IntQ
  {\TypeInter{\cdot}}: \Types \to \etaInter \to \Pd(\Domain)$
  be an interpretation of types parametric in a well-kinded
  interpretation of variables.
  The associated \emph{extensional interpretation} of types is the unique function
  $\ExtInter(\cdot): \Types \to \etaInter \to \Pd(\ExtInter_\Domain)$
  such that:

\noindent
   \(\begin{array}{rl}
    \ExtInter(\Empty)_\eta
    &= \emptyset \\   
    \ExtInter(\alpha)_\eta
    &= \eta(\alpha) \\
    \ExtInter(b)_\eta
    &= \ConstantsInBasicType(b)\\
    \ExtInter(\neg t)_\eta
    &= \ExtInter_\Domain \setminus \ExtInter(t)_\eta\\
    \ExtInter(t_1 \lor t_2)_\eta
    &= \ExtInter(t_1)_\eta \cup \ExtInter(t_2)_\eta\\
    \ExtInter(t_1 \to t_2)_\eta
    &= \raisebox{-.5pt}{$\Pd(\overline{\parbox[][10.7pt][c]{48pt}{$\TypeInter{t_1}_\eta\times\overline{\parbox[][8.8pt][c]{18pt}{$\TypeInter{t_2}_\eta$}}$}}\,)$}
    %% \Pd(\overline{%\IntQ
    %% {\TypeInter{t_1}_\eta} \times
    %% \overline{%\IntQ
    %% {\TypeInter{t_2}_\eta}}})
    \end{array}
    \begin{array}{rl}
    \ExtInter(\R)_\eta
    = \left\{
      \begin{array}{ll}\bigcup_{\drow \in \eta(\rho)}
         \left(\prodc{\ell \in \fin(\R)} \IntF{\TypeInter{\R(\ell)}}_\eta \pfconcat \drow \right)
    &\text{if $\tail(\R) = \rho$}\\
      \prodc{\ell \in \Labels} \IntF{\TypeInter{\R(\ell)}}_\eta &\text{otherwise}
      \end{array}\right.
      \end{array}
\)

\noindent
where

\(\begin{array}{rll}
   \IntF{\TypeInter{t}}_\eta &= %\IntQ
   {\TypeInter{t}}_\eta & \text{if } t\not=\neg t'
   \text{ and } t\not= t_1\vee t_2\qquad\qquad\\
   \IntF{\TypeInter{\fvar}}_\eta &= \eta(\fvar)\\
    \IntF{\TypeInter{\Undef}}_\eta &= \{\Undef\}
  \end{array}\begin{array}{rll}  
    \IntF{\TypeInter{\tau_1\lor\tau_2}}_\eta &=\IntF{\TypeInter{\tau_1}}_\eta\cup\IntF{\TypeInter{\tau_2}}_\eta \\
    \IntF{\TypeInter{\neg\tau}}_\eta &=
   (\ExtInter_\Domain\cup\{\Undef\}) \setminus  \IntF{\TypeInter{\tau}}_\eta
   \end{array}\)
\end{definition}    
Notice that the induction used in the definition is well-founded
thanks to the contractivity condition in the definition of types and
the fact that field-types are inductively defined.

The extensional interpretation is defined with respect to some domain
$\Domain$ and interpretation $\TypeInter .$, and maps types into a
domain $\ExtInter_\Domain$ that contains $\Domain$, 
constants $\Constants$ to interpret basic types,
sets of binary relations $\Pd(\Domain \times \Domain_\Omega)$ to
interpret function types, and quasi constant functions
$\Labels \qcfun \Domain_\Undef$ to interpret record types. The fact
that functions are binary relations that can yield a distinguished
element $\Omega$ (which, intuitively, represents a type error) is a
standard technique of semantic subtyping to avoid $\Any\to\Any$ to be a supertype  of
all function types: since it does not play any specific role in our
work we will not further
comment on it (see~\cite{frisch08} for a detailed explanation
or~\citet[Section 3.2]{castagna23a} for a shorter one).

The definitions for the extensional interpretation given on the right-hand side in \cref{d:extint}
 are the same as those by~\citet{castagna11}. They state that the
 empty type is interpreted as the empty set, the
 interpretation of the type variables is given by $\eta$, that unions
 and negations are interpreted as set-theoretic unions and
 complements, and that functions types are interpreted as sets of
 binary relations whose output is in the codomain if the input is in
 the domain.

The novelty of our definition is the interpretation of record
types given on the left-hand side. There are two cases. The easy case is when the tail  of the
record type is either $\crecsign$ or $\orecsign$: in that case the
interpretation of the record type is the set of all quasi constant
functions in $\Labels\qcfun \Pd(\Domain_\Undef)$ that map a label
$\ell$ into an element of the interpretation of $\R(\ell)$ (recall
that for $\ell\not\in\fin(\R)$, $\R(\ell)$ is $\Undef$
for $\tail(\R)=\crecsign$ and $\Any\lor\Undef$ for $\tail(\R)=\orecsign$).
If instead $\tail(\R)$ is a row variable $\rho$, then $\Labels$ is
partitioned in two, the sets $\fin(\R)$ and---by well-kindedness---$\dom(\rho)$, and the interpretation of $\R$ will be the set of
quasi-constant functions in $\Labels\qcfun\Domain_\Undef$ obtained by
unioning two partial functions: a function
in $\prodc{\ell \in \fin(\R)} \IntF{\TypeInter{\R(\ell)}}_\eta$ for the $\fin(\R)$ labels of $\Labels$, and a
function in $\eta(\rho)$ for the remaining labels of $\Labels$. There
is a caveat: fields can map labels both into values and
$\Undef$. Therefore, the interpretation of field-types must be
slightly different from that of types, since it must map $\Undef$ into
$\{\Undef\}$ and the negation of a field-type is the complement
with respect to $\Domain_\Undef$, rather than $\Domain$: the $\IntF{\TypeInter .}$ does just that.


Given a domain $\Domain$ and a set-theoretic interpretation of the
types into this domain, they form a \emph{model} if the interpretation
and the associated extensional interpretation have the same zeros:
\begin{definition}[Model]\label{def:model}
Let $\Domain$ be a domain and
$%\IntQ
{\TypeInter{\cdot}}: \Types \to \etaInter \to \Pd(\Domain)$. The
 pair $(\Domain,%\IntQ
 {\TypeInter{\cdot}})$ is a \emph{model} if and only, if for
 all $t\in\Types$ and $\eta\in\etaInter$, 
 $%\IntQ
 {\TypeInter{t}}_\eta=\emptyset\iff\ExtInter(t)_\eta=\emptyset$.
 \end{definition}
Every model induces a subtyping relation on types\footnote{Actually,
a model must be convex: see~\citet{castagna11}. We omit this detail
since it is not relevant to our presentation.}:

\begin{definition}[Subtyping]\label{def:frischsubtyping}
  If $(\Domain,%\IntQ
  {\TypeInter{\cdot}})$
  is a model, then it induces a subtyping relation defined as follows:
  \centerline{$t_1 \leq t_2 \iffdef \forall\eta.
    %\IntQ
    {\TypeInter{t_1}_\eta} \subseteq %\IntQ
    {\TypeInter{t_2}_\eta}$
  \phantom{follows:}}
\end{definition}
As explained by \citet[Section 2.6]{frisch04}, the interest of defining of a \emph{model} is that we can work
with the interpretation of the model ``\emph{as if}'' the interpretation
of the type
constructors (in particular, the function type constructor) were defined as their
extensional interpretation. So when deducing the properties for the
subtyping relation of a model---and just for the subtyping
relation---we can assume that \raisebox{-.5pt}{$\Pd(\overline{\parbox[][10.7pt][c]{48pt}{$\TypeInter{t_1}_\eta\times\overline{\parbox[][8.8pt][c]{18pt}{$\TypeInter{t_2}_\eta$}}$}}\,)$},
%% $\TypeInter{t_1 \to t_2}_\eta= \Pd(\overline{
%%     {\TypeInter{t_1}_\eta} \times
%%     \overline{
%%     {\TypeInter{t_2}_\eta}}})$,
even if this is impossible for cardinality reasons.    

\Cref{def:model} specifies which characteristics a model must
have to induce a subtyping relation (that behaves ``\emph{as if}''), but it does not define any
particular model nor, thus, any particular subtyping relation. In what follows
we define a concrete interpretation domain $\Domain$ (whose elements
are defined by induction) and two specific interpretations, and prove
that they satisfy the conditions to be  models, since they both have
the same zeros as the extensional interpretation (of one of them). This
yields two equivalent definitions of a concrete subtyping relation we
are going to use in the rest of this presentation.
We will define:
\begin{itemize}
  \item An interpretation $\IntQ{\TypeInter{t}_\eta}$ parameterized by an assignment $\eta$,
    for which subtyping $t_1 \IntQ{\leq} t_2$ is defined as
    $\forall\eta.\IntQ{\TypeInter{t_1}_\eta} \subseteq \IntQ{\TypeInter{t_2}_\eta}$;
    (the index $q$ stands for \emph{\textbf{q}uantified}, since subtyping is
    quantified on all variable interpretations);
  \item An interpretation of types directly into sets $\TypeInter t$, that avoids
    quantification over $\eta$, and for which subtyping $t_1 \leq t_2$ is defined
    directly as $\TypeInter{t_1} \subseteq \TypeInter{t_2}$ (notice
    the absence of a variable interpretation argument $\eta$).
\end{itemize}

The interpretation of types is mutually recursive with interpretations of rows and
field-types.
Both of these will also give rise to subtyping relations.
We will use the same notation $\leq$ for the relations in $\Types \times
\Types$, $\Types_\Undef \times \Types_\Undef$ and
$\Rows \times \Rows$.

%% \begin{definition}[Interpretation Domain]\label{def:interpretation}
%%   As \emph{interpretation domain} $\Domain$ for types, we take the set of finite terms $d$
%%   produced inductively by the following grammar, where $c$ ranges over the set
%%   $\Constants$ of constants, $\ell$ over the set $\Labels$ of labels, and $V$ over sets of variables contained
%%   in $\Vars=\typeVars\cup\fldVars\cup\rowVars$.
%%   The interpretation domain $\Domain_\Undef$ for fields (resp. $\Domainrow$ for
%%   rows) is the set of terms $\dundef$ (resp. $\drow$).
%%   \begin{align*}
%%     d & \Coloneqq  c^V \mid \{(d, \domega), \dots, (d, \domega)\}^V
%%     \mid \domrec{\drow}^V
%%       & \dom(\drow) = \Labels \\[-1.3mm]
%%     \drow & \Coloneqq \domrow{\ell_1 = \dundef, \dots, \ell_n = \dundef}{L}^V
%%           & L \in \Pf(\Labels\setminus\{\ell_1,...,\ell_n\}) \\[-1.3mm]
%%     \domega & \Coloneqq d \mid \Omega\\[-1.3mm]
%%     \dundef & \Coloneqq d \mid \Undef^V
%%   \end{align*}
%%   We use $\dterm$ for an element that is either $d$, $\drow$ or $\dundef$.
%%   We define $\dom(\domrow{(\ell = \dundef_\ell)_{\ell \in L_1}}{L_2}^V) =
%%   \Labels \setminus L_2$. We use $\Tag(\dterm)$ to denote the set of
%%   variables indexing $\dterm$, that is, $\Tag(c^V)=\Tag(\{(d, \domega), \dots, (d, \domega)\}^V)=\Tag(\domrec{\drow}^V)=\Tag(\domrow{\ell_1 = \dundef, \dots, \ell_n = \dundef}{L}^V)=\Tag(\Undef^V) =V$.
%% \end{definition}
%% The intuition behind this definition is simple. The elements of
%% the domain are either constants, or finite binary relations (which
%% are finite approximations of functions), or rows. The last ones
%% are \emph{partial} quasi-constant functions in
%% $\Labels\pqcfun\Domain_\Undef$ with default value $\Undef$. More
%% precisely the row $\domrow{\ell_1 = \dundef_1, \dots, \ell_n = \dundef_n}{L}$
%% is the quasi-constant function $\qcf{\ell_1
%% = \dundef_1, \dots, \ell_n = \dundef_n,\wild=\Undef}$ in $(\Labels\setminus
%% L)\qcfun\Domain_\Undef$. When a row is total on $\Labels$, then it can
%% be wrapped in a $\domrec{}$ constructor yielding (the interpretation
%% of) a record value (the inverse operation is given in \cref{def:row}). Furthermore, all the elements are indexed by
%% a finite set of variables ranged over by $V$. This is a standard technique introduced
%% by~\citet{gesbert15} to interpret type variables (cf.~\cref{def:indint}), while ensuring that the model
%% we obtain is \emph{convex} in the sense of~\citet{castagna11}. The
%% domain of \cref{def:interpretation} is the
%% one by~\citet{gesbert15}, but where records and rows replace pairs.

%% \begin{definition}\label{def:row}
%%   Let $\R = \rec{(\ell = \tau_\ell)_{\ell \in L}}{\tl}$.
%%   We define $\rectorow\R = \row{(\ell = \tau_\ell)_{\ell \in L}}{\tl}{\emptyset}$.
%%   We extend this definition homomorphically to Boolean combinations of
%%   record type atoms.
%% \end{definition}

%% We have now all ingredients needed to define our first interpretation
%% for the types:

%% \begin{definition}[Interpretation of Types and Rows as Sets]
%%   \label{def:indint}%
%%   Let $\Domain$ be the domain of~\cref{def:interpretation} and $\Types$ the
%%   types of \cref{def:types}. We define a binary predicate $(\dterm : \tterm)$
%%   (“the element $\dterm$ belongs to $\tterm$”) on $\Domain\times\Types \cup
%%   \Domain_\Undef \times \Types_\Undef \cup \Domainrow \times \Rows$
%%   by induction on the pair $(\dterm, \tterm)$ ordered lexicographically.
%%   The predicate is only defined if $\dterm$ is coherent with the kind of
%%   $\tterm$:
%%   $\dterm = d$ if $\tterm = t$, $\dterm = \dundef$ if $\tterm = \tau$, and
%%   $\dterm = \drow$ if $\tterm = \rw$ and $\dom(\dterm) = \dom(\rw)$.
%%   \begin{itemize}
%%     \item On types:\vspace{-2mm}
%%       \begin{align}
%%         (d : \alpha)
%%         &= \alpha \in \Tag(d) \label{due}\\[-1.5mm]
%%         (c^V : b)
%%         &= c \in \ConstantsInBasicType(b) \\[-1.5mm]
%%         (\{(d_1, \domega_1), \dots, (d_n, \domega_n)\}^V : t_1 \to t_2)
%%         &= \forall i \in [1.. n] . \:
%%         \mathsf{if} \: (d_i : t_1) \mathrel{\mathsf{then}} (\domega_i : t_2) \\[-1.5mm]
%%         (\domrec{\drow}^V:\R)
%%         &= (\drow:\rectorow{\R})
%%       \end{align}
%%     \item On fields:\vspace{-2mm}
%%       \begin{align}
%%         (\dundef : \fvar) &= \fvar \in \Tag(\dundef)
%%         & (\Undef^V : \Undef) &= \mathsf{true}
%%       \end{align}
%%     \item On atomic rows:\vspace{-2mm}
%%       \begin{align}
%%         (\domrow{(\ell = \dundef_\ell)_{\ell \in L_1}}{L_2}^V:\rw)
%%         &= (\forall \ell \in L_1. (\dundef_\ell:\rw(\ell))) \textand
%%         (\forall\ell \in \dom(\rw)\setminus L_1. (\Undef^\emptyset:\rw(\ell)))\label{sette}\\[-1.8mm]
%%         &\phantom{=}\ \textand \tail(\rw) = \rho \implies \rho \in V\label{otto}
%%       \end{align}
%%     \item On types, fields and rows (where $\tterm_1$ and $\tterm_2$ are of the same kind):\vspace{-2mm}
%%       \begin{align}
%%         (\dterm : \tterm_1 \lor \tterm_2)  &= (\dterm : \tterm_1) \textor (\dterm : \tterm_2) \\[-1.5mm]
%%         (\dterm : \lnot \tterm)  &= \mathsf{not} \: (\dterm : \tterm)
%%         \text{ and the kinds of $\dterm$ and $\tterm$ correspond} \\[-1.5mm]
%%         (\dterm : \tterm)  &= \mathsf{false} \hspace*{2cm} \text{otherwise}
%%       \end{align}
%%   \end{itemize}
%%   We define the interpretation $\TypeInter{\cdot} : \Types \to \Pd(\Domain)$
%%   as $\TypeInter{t} = \{d \in \Domain \mid (d : t)\}$,
%%   the interpretation $\IntF{\TypeInter{\cdot}} : \Types_\Undef \to \Pd(\Domain_\Undef)$
%%   as $\IntF{\TypeInter{\tau}} = \{\dundef \in \Domain_\Undef \mid (\dundef:\tau)\}$, and
%%   the interpretation $\IntR{\TypeInter{\cdot}} : \Rows \to \Pd(\Domainrow)$
%%   as $\IntR{\TypeInter{\rw}} = \{\drow \in \Domainrow \mid (\dbar:\rw)\}$.
%% \end{definition}
%% The interpretation of \cref{def:indint} is mostly the same as the one by~\citet{gesbert15}, where the
%% interpretation of a type variables $\alpha$ is the set of all elements
%% that are tagged by $\alpha$ (see \cref{due}). The only difference with
%% respect to \cite{gesbert15} is
%% the interpretation of rows and, thus, of record types. Lines \eqref{sette} and \eqref{otto} define when a row element is in the
%% interpretation of a row  $r$: it requires that all the components of
%% the row element are in the interpretations of the types specified by
%% $r$ (line~\eqref{sette}) and if the tail of $r$ is a row variable,
%% then it must index the row element (line~\eqref{otto}).

This interpretation in \cref{def:indint} induces a subtyping relation that it is easy to work with, since it got rid of the
interpretation $\eta$ for the variables. We can consider the
interpretation $\TypeInter{\cdot} : \Types \to \Pd(\Domain)$ as a
function in   $\Types  \to \etaInter\to \Pd(\Domain)$ that is constant
on its second argument: if we apply \cref{def:frischsubtyping} to it, then  the subtyping relation is
defined as simply as
$t_1 \leq t_2 \iffdef \TypeInter{t_1} \subseteq \TypeInter{t_2}$.
But getting rid of $\eta$ makes it difficult to prove that this interpretation is a model and, thus,
that when considering the properties of this subtyping relation, we can work ``as if'' the interpretation
of type constructors were as in the extensional interpretation. To overcome this difficulty we define a second
interpretation, on the same domain, but this interpretation disregards the indexes
of the elements and uses an assignment $\eta$ to interpret the variables.
\begin{definition}[Parametrized intepretation of types and rows]
  \label{def:indinteta}%
  We define a ternary predicate $\IntQ{(\dterm : \tterm)_\eta}$
  (``the element $\dterm$ belongs to $\tterm$ under assignment $\eta$''),
  by induction on the pair $(\dterm, \tterm)$ ordered lexicographically.
  The only differences with the predicate $(\dterm : \tterm)$ (apart from
  recursive calls to the appropriate predicate), are:
  \begin{align*}
    \IntQ{(d : \alpha)_\eta}
    &= d \in \eta(\alpha) \\
    \IntQ{(\dundef : \fvar)_\eta}
    &= \dundef \in \eta(\fvar) \\
    \IntQ{(\domrow{(\ell = \dundef_\ell)_{\ell \in L_1}}{L_2}^V:\rw)_\eta}
    &= (\forall \ell \in L_1. \IntQ{(\dundef_\ell:\rw(\ell))_\eta})
    \textand (\forall \ell \in \dom(\rw) \setminus L_1.
    \IntQ{(\Undef^\emptyset:\rw(\ell))_\eta}) \\[-1.5mm]
    &\phantom{=}\ \textand \tail(\rw) = \rho \implies
    \domrow{(\ell = \dundef_\ell)_{\ell \in L_1 \cap
    \dom(\rho)}}{\Labels{\setminus}\dom(\rho)}^V \in \eta(\rho)
  \end{align*}
  We define the interpretations $\IntQ{\TypeInter{\cdot}_\eta}$,
  $\IntQF{\TypeInter{\cdot}_\eta}$ and $\IntQR{\TypeInter{\cdot}_\eta}$ as expected.
\end{definition}
While the interpretation of type and field variables is
straightforwardly given by $\eta$, the interpretation of row variables
is less evident.
The first line of the interpretation of a row is the same as
in \cref{def:indint}: in both definitions this line deals with the case when
the tail of $r$ is not a row variable.
The second line covers the case for $\tail(r)=\rho$:  it checks that $\drow \in \eta(\rho)$, where $\drow$
is obtained by restricting the quasi-constant function on the left to the domain of
$\rho$.

Our goal is to prove that both interpretations give a model of
types. Formally, this corresponds to proving the following theorem:
\begin{theorem}
Let $\ExtInter(\cdot)$ be the extensional interpretation of
$\IntQ{\TypeInter{.}}$. For all $t \in \Types$:
\begin{equation}
  \label{eq:same_zeros}%
  (\forall \eta.\ExtInter(t)_\eta = \emptyset)
  \iff (\forall \eta.\IntQ{\TypeInter{t}_\eta} = \emptyset)
  \iff \TypeInter{t} = \emptyset
\end{equation}
\end{theorem}

\begin{proof}(Hint)
  Given an element $d \in \Domain$, we show
  $d \in \ExtInter(t)_\eta \iff d \in \IntQ{\TypeInter{t}_\eta} \iff d \in
  \TypeInter{t}$ by lexicographic induction on $(d,t)$.
  The proof of the leftmost equivalence is straightforward.
  For the second equivalence, we introduce a canonical assignment $\hat\eta$
  defined as
  $\hat\eta(\alpha)
  = \{ d \in \Domain \mid \alpha \in \Tag(d) \}$,
  $\hat\eta(\fvar)
  = \{ \dundef \in \Domain_\Undef \mid \fvar \in \Tag(\dundef) \}$ and
  $\hat\eta(\rho) 
  = \{ \drow \in \Domainrow \mid \dom(\drow) = \dom(\rho) \textand \rho \in
  \Tag(\drow) \}$.
  Then, we show that $d \in \IntQ{\TypeInter{t}_\eta}
  \iff d \in \IntQ{\TypeInter{t}_{\hat\eta}}
  \iff d \in \TypeInter{t}$.
  All details are given in \cref{app:subtyping}.
\end{proof}
The leftmost ``iff'' proves that $(\Domain,\IntQ{\TypeInter{.}})$ is a
model, while the rightmost one proves that the subtyping relation
induced by $\TypeInter{.}$ is the same as the one induced by the model
$\IntQ{\TypeInter{.}}$ (since
$\forall \eta.\IntQ{\TypeInter{s}_\eta} \subseteq\IntQ{\TypeInter{t}_\eta} \iff\forall \eta.\IntQ{\TypeInter{s}_\eta} \cap
(\Domain{\setminus}\IntQ{\TypeInter{t}_\eta}) = \emptyset \iff\forall \eta.\IntQ{\TypeInter{s{\wedge}\neg
t}_\eta} = \emptyset \iff \TypeInter{s{\wedge}\neg t} = \emptyset \iff \TypeInter{s}\subseteq\TypeInter{t}$).


==> tuples.tex <==
\subsection{Representation of record types}

We introduce a notation of records as tuples.
With this representation, record types can be represented as finite unions of
tuples.

A preliminary step is to introduce a notation for \emph{quasi-open} records:
\[
  \qorec{(\ell = \tau_\ell)_{\ell \in L}}
  \eqdef \orec{(\ell = \tau_\ell)_{\ell \in L}} \wedge \neg\crec L
\]
These are records where one of the elements not in $L$ must be defined.
%Later on, we will also use this notation for quasi-open rows:
%\[
%  \qorow{(\ell = \tau_\ell)_{\ell \in L'}}{L}
%  \eqdef \orow{(\ell = \tau_\ell)_{\ell \in L'}}{L} \wedge \neg\crow{L'}{L}
%\]
This notation allow us to represent the negation of any non-polymorphic record
in a positive form.
Indeed, observe that $
\neg\crec L \wedge \orec{} \simeq \qorec L$
and $\neg\qorec L \wedge \orec{} \simeq \crec L$.
So that, for instance, we can rewrite
\[
  \orec{} \wedge \neg\crec{(\ell = \tau_\ell)_{\ell \in L}}
  \ \text{ to }\ 
  \bigvee_{\ell \in L} \orec{\ell = \neg\tau_\ell} \vee \qorec L
\]
instead of
$\orec{} \wedge (\bigvee_{\ell \in L} \orec{\ell = \neg\tau_\ell} \vee
\neg\crec L)$.
We define $\Def(\R) \eqdef \Any \lor \Undef$ for $\R$ quasi-open.

In the new representation, the name $\monotl$ ranges over $\orecsign,
\crecsign$ or $\qorecsign$.
Let $V_p, V_n \subset \rowVars$.
We define
\begin{equation}
  \label{eq:recdef}%
  \rrec{(\tau_\ell)_{\ell \in L}}{\monotl}{V_p}{V_n}
  = \rec{(\ell = \tau_\ell)_{\ell \in L}}{\monotl}
  \wedge \bigwedge_{\rho \in V_p} \prec{\Labels{\setminus}\dom(\rho)}{\rho}
  \wedge \bigwedge_{\rho \in V_n} \neg\prec{\Labels{\setminus}\dom(\rho)}{\rho}
\end{equation}
We use the name $\RR$ to range over those atoms.
For the record defined in \eqref{eq:recdef}, we have $\fin(\RR) = L$ and define
$\tail(\RR) = \monotl$.
We define $\RR(\ell) = \rec{(\tau_\ell)_{\ell \in L}}{\monotl}(\ell)$.

\begin{lemma}
  The following holds.
  \begin{equation}
    \label{eq:empty_rec}%
      \rrec{(\tau_\ell)_{\ell \in L}}{\monotl}{V_p}{V_n} \simeq \Empty
      \iff \exists \ell {\in} L. \tau_\ell \simeq \Empty
      \textor V_p \cap V_n \neq \emptyset
  \end{equation}

  \begin{equation}
    \label{eq:inter_rec}%
    \begin{split}
      \rrec{(\tau_\ell^1)_{\ell \in L}}{\monotl_1}{V_p^1}{V_n^1} \wedge
      \rrec{(\tau_\ell^2)_{\ell \in L}}{\monotl_2}{V_p^2}{V_n^2} \\
      = \begin{cases}
        \rrec{(\tau_\ell^1 \wedge \tau_\ell^2)_{\ell \in L}}
        {\monotl_1}{V_p^1 \cup V_p^2}{V_n^1 \cup V_n^2}
      &\text{if } \monotl_1 = \monotl_2 \textor \monotl_2 = \orecsign;\\
      \rrec{(\tau_\ell^1 \wedge \tau_\ell^2)_{\ell \in L}}
      {\monotl_2}{V_p^1 \cup V_p^2}{V_n^1 \cup V_n^2}
      &\text{ if } \monotl_1 = \orecsign;\\
        \Empty &\text{otherwise.}
      \end{cases}
    \end{split}
  \end{equation}

  \begin{equation}
    \label{eq:minus_rec}%
    \begin{split}
      \rrec{(\tau_\ell)_{\ell \in L}}{\monotl}{V_p}{V_n} \typediff
      \rrec{(\tau'_\ell)_{\ell \in L}}{\monotl'}{V'^+}{\emptyset}
      = \begin{cases}
        \RR \vee \rrec{(\tau_\ell)_{\ell \in L}}{\qorecsign}{V_p}{V_n}
        &\text{if } \monotl \neq \crecsign \textand \monotl' =
        \crecsign;\\
        \RR &\text{otherwise}
      \end{cases}\\
      \text{with } \RR =
      (\bigvee_{\ell_0 \in L} \rrec{(\tau_\ell^{\ell_0})_{\ell \in
      L}}{\monotl}{V_p}{V_n})
      \vee \bigvee_{\rho \in V'^+}
      \rrec{(\tau_\ell)_{\ell \in L}}{\monotl}{V_p}{V_n \cup \{\rho\}}
    \end{split}
  \end{equation}
  for $\monotl' \in \{\crecsign,\orecsign\}$ and
  where $\tau_\ell^{\ell_0}$ is $\tau_\ell \typediff \tau'_\ell$ if $\ell_0 =
  \ell$ and $\tau_\ell$ otherwise.
\end{lemma}

\begin{proof}
  In the following, let
  $\RR = \rrec{(\tau_\ell)_{\ell \in L}}{\tl}{V_p}{V_n}$.

  We start with~\eqref{eq:empty_rec}.
  First, it is easy to see that if one the conditions on the right does not
  hold, then $\RR$ is empty.
  Now, suppose that $\RR$ is empty and show that one of the following hold:
  $\exists \ell \in L. \tau_\ell \leq \Empty$ or $V_p \cap V_n = \emptyset$.

  Let $N_\Vars = \{\prec{\Labels{\setminus}\dom(\rho)}{\rho} \mid \rho \in V_n\}$.
  Let $t = \crec L$ if $\tl = \qorecsign$ and $t = \Empty$ otherwise.
  The type $\RR$ is equivalent to $\RR' \wedge \neg t$, with $\RR' \eqdef \RR$
  when $\tl \neq \qorecsign$ and $\RR' \eqdef \rec{(\tau_\ell)_{\ell \in
  L}}{\orecsign}{V_p}{V_n}$ when $\tl = \qorecsign$.
  Let $N = \{t\} \cup N_\Vars$.
  By \cref{l:subtyping}, since $\RR$ is empty, for any $\iota:N \to L \cup
  \{\_\}$ one of the two following statements holds:
  \begin{enumerate}
    \item $\exists \ell \in L. \tau_\ell \leq \bigvee_{n \in \iota^{-1}(\ell)}
      \Any \lor \Undef$ or
    \item $\iota^{-1}(\_) \cap V_p \neq \emptyset$.
  \end{enumerate}
  Indeed, the second condition of \cref{l:subtyping} never holds, either, in
  the case $\tl = \qorecsign$ because $\Def(\orec{(\tau_\ell)_{\ell \in L}})
  = \Any \lor \Undef$ while $\Def(t) = \Undef$,
  or, in the cases $\tl = \orecsign$ and $\tl = \crecsign$ because $\Def(t) = \Empty$.
  Now, take the function $\iota$ that associates $\_$ to every element of $N$.
  The first statement becomes $\exists \ell. \tau_\ell \leq \Empty$ because
  $\iota^-{1}(\ell)$ is empty for all $\ell$.
  The second statement becomes $V_n \cap V_p \neq \emptyset$.

  We now consider~\eqref{eq:inter_rec}.
  Let $\RR' = \rrec{(\tau'_\ell)_{\ell \in L}}{\tl'}{V'^+}{V'^-}$.
  \begin{align*}
    \RR \land \RR'
    &= \rec{(\ell = \tau_\ell)_{\ell \in L}}{\tl}
    \wedge \bigwedge_{\rho \in V_p} \prec{L_\rho}{\rho}
    \wedge \bigwedge_{\rho \in V_n} \neg\prec{L_\rho}{\rho}\\
    &\quad\wedge \rec{(\ell = \tau'_\ell)_{\ell \in L}}{\tl'}
    \wedge \bigwedge_{\rho \in V'^+} \prec{L_\rho}{\rho}
    \wedge \bigwedge_{\rho \in V'^-} \neg\prec{L_\rho}{\rho}\\
    &\simeq \orec{(\ell = \tau_\ell \wedge \tau'_\ell)_{\ell \in L}}
    \wedge \rec L \tl
    \wedge \rec L {\tl'}
    \quad\wedge \bigwedge_{\rho \in V_p \cup V'^+} \prec{L_\rho}{\rho}
    \wedge \bigwedge_{\rho \in V_n \cup V'^-} \neg\prec{L_\rho}{\rho}
  \end{align*}
  If $\tl = \tl'$ or $\tl' = \orecsign$, we have $\rec L \tl \wedge
  \rec
  L {\tl'} = \rec L \tl$.
  If $\tl = \orecsign$, we have $\rec L \tl \wedge \rec L {\tl'} =
  \rec L {\tl'}$.
  In the other cases, we have $\rec L \tl \wedge \rec L {\tl'} =
  \Empty$, so the whole type is empty.

  We finally consider~\eqref{eq:minus_rec}.
  Let $\RR' = \rrec{(\tau'_\ell)_{\ell \in L}}{\monotl'}{V'^+}{\emptyset}$ with $\monotl'
  \neq \qorecsign$.
  \begin{align*}
    \RR \typediff \RR'
    &= \RR \wedge \neg\Big(\rec{(\ell = \tau_\ell)_{\ell \in L}}{\monotl'} \wedge
    \bigwedge_{\rho \in V'^+} \prec{L_\rho}{\rho}\Big)\\
    &\simeq \RR \wedge \neg\Big(\bigwedge_{\ell \in L} \orec{\ell = \tau_\ell} \wedge
    \rec L {\monotl'} \wedge
    \bigwedge_{\rho \in V'^+} \prec{L_\rho}{\rho}\Big)\\
    &\simeq \RR \wedge \Big(\bigvee_{\ell \in L} \orec{\ell = \neg\tau_\ell} \vee
    \neg\prec L {\monotl'} \vee
    \bigvee_{\rho \in V'^+} \neg\prec{L_\rho}{\rho}\Big)\\
    &\simeq (\bigvee_{\ell \in L} \RR \wedge \orec{\ell = \neg\tau_\ell}) \vee
    (\RR \wedge \neg\rec L {\monotl'}) \vee
    \bigvee_{\rho \in V'^+} (\RR \wedge \neg\prec{L_\rho}{\rho})\\
  \end{align*}
  We obtain $\bigvee_{\ell_0 \in L} \rrec{(\tau_\ell^{\ell_0})_{\ell \in
  L}}{\monotl}{V_p}{V_n}$ from
  $\bigvee_{\ell \in L} (\RR \wedge \orec{\ell = \neg\tau_\ell})$ directly,
  as well as $\bigvee_{\rho \in V'^+} \rrec{(\tau_\ell)_{\ell \in
  L}}{\monotl}{V_p}{V_n \cup \{\rho\}}$ from
  $\bigvee_{\rho \in V'^+} (\RR \wedge \neg\prec{L_\rho}{\rho})$.
  Moreover, the type $\RR \wedge \neg\rec L {\monotl'}$ is equal to:
  \[
    \rec{(\ell = \tau_\ell)_{\ell \in L}}{\monotl}
    \wedge \bigwedge_{\rho \in V_p} \prec{L_\rho}{\rho}
    \wedge \bigwedge_{\rho \in V_n} \neg\prec{L_\rho}{\rho}
    \wedge \neg\rec L {\monotl'}
  \]
  If $\tl' = \crecsign$ and $\tl \neq \crecsign$,
  $\rec L \tl \wedge \neg\rec L {\monotl'} = \qorec L$.
  In all other cases, in particular $\tl' = \orecsign$, the type is empty.
\end{proof}

\begin{lemma}
  Let $t \leq \orec{}$ and $t \nleq \Empty$.
  Let $L \in \Pf(\Labels)$ such that $\fin(t) \subseteq L$.
  Then, there exists a finite set $S$ of non-empty types of the form
  $\rrec{(\tau_\ell)_{\ell \in L}}{\monotl}{V_p}{V_n}$ such that
  \[
    t \simeq \bigvee_{\RR \in S}
    \rrec{(\tau_\ell)_{\ell \in L}}{\monotl}{V_p}{V_n}
  \]
\end{lemma}
\begin{proof}
  Since $t \leq \orec{}$, then $t$ is equivalent to
  $\bigvee_{i \in I} (\bigwedge_{\R \in P_i} \R \wedge \bigwedge_{\R \in N_i}
  \neg\R)$, where the $\R$'s are atomic rec types.
  Atomic rec types can be represented as
  $\rrec{(\tau_\ell)_{\ell \in L}}{\monotl}{V_p}{\emptyset}$ with $\monotl \in
  \{\orecsign\,,\crecsign\}$.
  By applications of~\eqref{eq:inter_rec} we transform every
  $\bigwedge_{\R \in P_i} \R$ into a rec of the form
  $\rrec{(\tau_\ell)_{\ell \in L}}{\monotl}{V_p}{V_n}$.
  We conclude by iterating the difference of the records obtained at each step,
  starting with the one obtained from the positive occurences, and each rec
  in $N_i$.
  The tuple shape of the type is guaranteed by~\eqref{eq:minus_rec}.
  In the end, we simply remove empty types from $S$.
\end{proof}

\paragraph{Substitution}
If $\sigma(\rho) = \bigvee_{i \in I} \RR_i$ with
$\RR_i = \rrow{(\tau_\ell^i)_{\ell \in L'}}{\monotl_i}{V_p^i}{V_n^i}{L}$,
all non-empty, the following equality is satisfied:
\begin{equation}
  \prec{(\ell = \tau_\ell)_{\ell \in L}}{\rho}\sigma =
  \bigvee_{i \in I} \rrec
  {(\tau_\ell\sigma)_{\ell \in L}, (\tau_\ell^i)_{\ell \in L'}}
  {\monotl_i}{V_p^i}{V_n^i}
\end{equation}

\paragraph{Operations on records}

Let $t = \bigvee_{i \in I} \rrec{(\tau^i_{\ell})_{\ell \in L}}
{\monotl_i} {V_p^i} {V_n^i}$.
We can define:
$t.\ell = \bigvee_{i \in I} \tau^i_\ell$, because by the condition $t \leq \orec{\ell = \Any}$,
all $\tau^i_\ell$ are not optional nor undefined and $\ell \in L$.

\subsection{normalization procedure}

We can simplify the presentation of normalization in tallying by using the
representation as tuples, as in \cref{fig:nrules-recbis}.
\loic{Il manque l'ajout des $\rho.\ell$.}

\loic{Réécrire, on met $\orecsign$ pour une variable. Mettre aussi la définition
$\cutrowbis \rr L \Delta$ plus loin.}
We extend $\cutrow \rw L$ to
$\rw = \rrow{(\tau_\ell)_{\ell \in L_\circ}}{\monotl}{V_p}{V_n}{L'}$ by
\[
  \cutrow \rw L = \rrow{(\tau_\ell)_{\ell \in
  L_\circ{\setminus}L}}{\monotl'}{V_p'}{V_n'}{L' \cup L}
  \quad \text{with}
\]
\begin{itemize}
  \item $\monotl' = \orecsign$ if $\monotl = \qorecsign$ and $L \cap L'
    \nsubseteq L_\circ$, and $\monotl' = \monotl$ otherwise;
  \item $V_p' = \{\cutvar \rho L \mid \rho \in V_p\}$ and
  $V_n' = \{\cutvar \rho L \mid \rho \in V_n\}$.
\end{itemize}

The decomposition lemma is the following.
\begin{lemma}
  \label{l:optimised_decomposition}%
  Let $L$ be a finite set of labels,
  $\rr = \rrow{(\tau_\ell)_{\ell \in L_1}}{\monotl}{V_p}{V_n}{L_2}$.
  Let $V_p^\Delta = \{\rho \in V_p \mid L \cap \dom(\rho) \neq \emptyset\}$,
  similarly for $V_n^\Delta$.
  $\rr \leq \Empty$ \textit{iff}
  \[
    \exists\ell \in L \cap L_1. \tau_\ell \leq \Empty
    \textor \bigwedge_{\rho \in V_P^\Delta}
    \row{\Labels \setminus \dom(\rho)}{\rho}{L_2}
    \leq \bigvee_{\rho \in V_n^\Delta}
    \row{\Labels \setminus \dom(\rho)}{\rho}{L_2}
    \textor \cutrow \rr L \leq \Empty
  \]
\end{lemma}
\begin{proof}
  \loic{TODO (similaire à \cref{eq:empty_rec}).}
\end{proof}

\begin{figure}
  \begin{mathpar}
    \inferrule*[right=\rulename{Nsdnf}]
    {\normseq \Sigma {\{(\sdnf(\rw),\leq,\Empty)\}} \constrset
    \and \rw \neq \sdnf(\rw)}
    {\normseq \Sigma {\{(\dnf(\rw),\leq,\Empty)\}} \constrset}
    \and \inferrule*[right=\rulename{Nrow}]
    {\forall \ell \in L_1 \cap L.
      \normseq \Sigma {\{(\tau_\ell \leq \Empty)\}} {\constrset_\ell}\\\\
      \normseq \Sigma {\{(
          \cutrowbis {\rrow{(\tau_\ell)_{\ell \in L_1}}{\monotl}{V_p}{V_n}{L_2}} L \Delta
      \leq \Empty)\}} {\constrset_\rr} \\\\
      \normseq \Sigma {\{(
          \bigwedge_{\rho \in V_p^\Delta} \row{\Labels \setminus \dom(\rho)}{\rho}{L_2}
          \wedge \bigwedge_{\rho \in V_n^\Delta} \neg\row{\Labels \setminus \dom(\rho)}{\rho}{L_2}
      \leq \Empty)\}} {\constrset_\Delta}\\\\
      \rho \lightning_O V_p \cup V_n
      \and \rho \notin \Delta
      \and L = \Labels \setminus L_2 \setminus \dom(\rho) \neq \emptyset\\\\
      P_V^\Delta = \{\rho \in P_V \cap \Delta \mid \dom(\rho) \cap L \neq \emptyset\}
      \and N_V^\Delta = \{\rho \in N \cap \Delta \mid \dom(\rho) \cap L \neq \emptyset\}
    }
    {
      \normseq \Sigma
      {\{(\rrow{(\tau_\ell)_{\ell \in L_1}}{\monotl}{V_p}{V_n}{L_2}
      \leq \Empty)\}}
      {\constrset_\rr \sqcup \constrset_\Delta \sqcup \bigsqcup_{\ell \in L_1
    \cap L} \constrset_\ell} }
    \and \inferrule*[right=\rulename{Ntail-mono}]
    {
      V_p \cup V_n \subseteq \Delta
      \and \forall \ell \in L_1.
      \normseq \Sigma {\{(\tau_\ell \leq \Empty)\}} {\constrset_\ell}
    }
    {\normseq \Sigma {\{(\rrow{(\tau_\ell)_{\ell \in
      L_1}}{\monotl}{V_p}{V_n}{L_2},\leq,\Empty)\}}
    {\bigsqcup_{\ell \in L} \constrset_\ell}}
    \and \inferrule*[right=\rulename{Ntail-tlv}]
    {
      \constrset =
      {\begin{cases}
          \{\{(
              \rho, \leq,
              \neg \rrow{(\tau_\ell)_{\ell \in
              L_\circ}}{\monotl}{V_p{\setminus}\{\rho\}}{V_n}{L_2}
          )\}\}, &\text{if } \rho \in V_p\\
          \{\{(
              \rho, \geq,
              \rrow{(\tau_\ell)_{\ell \in L_\circ}}{\monotl}{V_p}{V_n{\setminus}\{\rho\}}{L_2}
      )\}\}, &\text{if } \rho \in V_n
  \end{cases}} \\\\
  \rho \lightning_O V_p \cup V_n
  \and \rho \notin \Delta
  \and \dom(\rho) = \Labels \setminus L_2
}
{\normseq \Sigma
  {\{(\rrow{(\tau_\ell)_{\ell \in L_1}}{\monotl}{V_p}{V_n}{L_2} \leq \Empty)\}}
\constrset}
\end{mathpar}
{\small Where $\rw$ in \rulename{Nsdnf} is a single normal form.}
\caption{Alternative normalization rules for rows}
\label{fig:nrules-recbis}
\end{figure}

Lemmes :
\begin{itemize}
  \item Soundness
  \item Termination
\end{itemize}

